Computational Complexity of Games and Puzzles

In this thesis, we survey techniques and results from the study of Complexity Theory and Games. We then apply these techniques to obtain new results for previously unstudied games. Our contributions in the games Hexiom, Cut the Rope, and Back to Bed may be helpful in further studies by exploiting structure common to several games. We also highlight some interesting paths for further study related to uncertainty that have yet to receive thorough study given their prevalence in today's games.

==> Chapters/IST-Thesis-MSc-Acknowledgments.tex <==
% #############################################################################
% Agradecimentos / Acknowledgments
% !TEX root = ../main.tex
% #############################################################################

I would like to thank my parents for their friendship, encouragement and caring over all these years, for always being there for me through thick and thin and without whom this project would not be possible. I would also like to thank my grandparents, aunts, uncles and cousins for their understanding and support throughout all these years.

Quisque facilisis erat a dui. Nam malesuada ornare dolor. Cras gravida, diam sit amet rhoncus ornare, erat elit consectetuer erat, id egestas pede nibh eget odio. Proin tincidunt, velit vel porta elementum, magna diam molestie sapien, non aliquet massa pede eu diam. Aliquam iaculis. 

Fusce et ipsum et nulla tristique facilisis. Donec eget sem sit amet ligula viverra gravida. Etiam vehicula urna vel turpis. Suspendisse sagittis ante a urna. Morbi a est quis orci consequat rutrum. Nullam egestas feugiat felis. Integer adipiscing semper ligula. Nunc molestie, nisl sit amet cursus convallis, sapien lectus pretium metus, vitae pretium enim wisi id lectus. 

Donec vestibulum. Etiam vel nibh. Nulla facilisi. Mauris pharetra. Donec augue. Fusce ultrices, neque id dignissim ultrices, tellus mauris dictum elit, vel lacinia enim metus eu nunc.

I would also like to acknowledge my dissertation supervisors Prof. Some Name and Prof. Some Other Name for their insight, support and sharing of knowledge that has made this Thesis possible.

Last but not least, to all my friends and colleagues that helped me grow as a person and were always there for me during the good and bad times in my life. Thank you.

To each and every one of you -- Thank you.

==> Chapters/IST-Thesis-MSc-Acronyms.tex <==
% #############################################################################
% This is the ACRONYMS Definition
% !TEX root = ../main.tex
% #############################################################################

\begin{acronym}[H.264/SVC]
    \acro{CNF}{Conjunctive Normal Form}
	\acro{SAT}{Satisfiability}
	\acro{TQBF}{True Quantified Boolean Formula}
	
	\acro{SMB}{Super Mario Bros.}
	
	\acro{NCL}{Non-Deterministic Constraint Logic}
	\acro{CSP}{Constraint Satisfaction Problem}
	
	\acro{P}{Deterministic Polynomial Time}
	\acro{NP}{Non-Deterministic Polynomial Time}
	\acro{PSPACE}{Deterministic Polynomial Space}
	\acro{NPSPACE}{Non-Deterministic Polynomial Space}
	\acro{EXPTIME}{Deterministic Exponential Time}
	\acro{NEXPTIME}{Non-Deterministic Exponential Time}
	\acro{ASP}{Another Solution Problem}
\end{acronym}

==> main.tex <==
% #############################################################################
% This is the MAIN DEFAULT DOCUMENT of the IST-Thesis MSc TEMPLATE.
% It is just used in order to LOAD the REAL MAIN FILE.
% Useful for online tools like writeLaTeX.com that expect a 'main.tex' document
% #############################################################################
% Please Choose:
\input{IST-Thesis-MSc-Main_Document.tex}
% \input{./IST-Thesis-MSc-Main_Document-PT}
% #############################################################################
% IST-Thesis-MSc
% Version 1.0, August 2014
% BY: Rui Santos Cruz, rui.s.cruz@tecnico.ulisboa.pt
% #############################################################################

==> tables_and_code/table_example.tex <==
% Table Example
\newcommand{\greyrow}{\rowcolor[rgb]{0.9,0.9,0.9}}
\newcommand{\whiterow}{\rowcolor[rgb]{1,1,1}}
\newcommand{\greycell}[1]{\multicolumn{1}{{>{\columncolor[rgb]{0.9,0.9,0.9}}c}}{#1}}
\newcommand{\lightgreycell}[1]{\multicolumn{1}{{>{\columncolor[rgb]{0.9,0.9,0.9}}c}}{#1}}
\newcommand{\mediumgreycell}[1]{\multicolumn{1}{{>{\columncolor[rgb]{0.8,0.8,0.8}}c}}{#1}}
\newcommand{\darkgreycell}[1]{\multicolumn{1}{{>{\columncolor[rgb]{0.7,0.7,0.7}}c}}{#1}}
\newcommand{\whitecell}[1]{\multicolumn{1}{{>{\columncolor[rgb]{1,1,1}}c}}{#1}}

\newcommand{\cellformatG}[1]{\multicolumn{1}{{>{\columncolor[rgb]{.9,.9,.9}}c}}{#1}}
\newcommand{\cellformatW}[1]{\multicolumn{1}{{>{\columncolor[rgb]{1,1,1}}c}}{#1}}
\newcommand{\cellformatlG}[1]{\multicolumn{1}{{|>{\columncolor[rgb]{.9,.9,.9}}c}}{#1}}
\newcommand{\cellformatlW}[1]{\multicolumn{1}{{|>{\columncolor[rgb]{1,1,1}}c}}{#1}}
\newcommand{\cellformatrG}[1]{\multicolumn{1}{{>{\columncolor[rgb]{.9,.9,.9}}c|}}{#1}}
\newcommand{\cellformatrW}[1]{\multicolumn{1}{{>{\columncolor[rgb]{1,1,1}}c|}}{#1}}
\newcommand{\cellformatlrG}[1]{\multicolumn{1}{{|>{\columncolor[rgb]{.9,.9,.9}}c|}}{#1}}
\newcommand{\cellformatlrW}[1]{\multicolumn{1}{{|>{\columncolor[rgb]{1,1,1}}c|}}{#1}}

\begin{table}[t]
\centering
\caption{Example table}
\label{table:table1}
\begin{tabular}{c c c c c c}
\hline
\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}\\
\cellformatrG{}&
\cellformatlG{\multirow{-2}{*}{\centering\bf \#Layers}} & 
\cellformatrG{\multirow{-2}{*}{\centering\bf \#Nets}} & 
\cellformatlG{\multirow{-2}{*}{\centering \#Nodes\Mark1}} & 
\cellformatrG{\multirow{-2}{1.8cm}{\centering Critical path}}&
\cellformatlG{\multirow{-2}{2cm}{\centering\bf Latency ($T_{iter}$)}}\\
\cellformatrG{\multirow{-3}{2.2cm}{\centering Benchmark: ANN}} &
\cellformatlG{\footnotesize $(1)$} & 
\cellformatrG{\footnotesize$(2)$} & 
\cellformatlG{\footnotesize$(3)=8\cdot(1)\cdot(2)$} & 
\cellformatrG{\footnotesize$(4)=4\cdot(1)$} & 
\cellformatlG{\footnotesize$(5)$}\\
\hline
\cellformatrW{A1} & \cellformatlW{\bf 3--1501} & \cellformatrW{       1   } & \cellformatlW{\bf 24--12008}  & \cellformatrW{\bf 12--6004} & \cellformatlW{    4}\\
\cellformatrW{A2} & \cellformatlW{    501    } & \cellformatrW{       1   } & \cellformatlW{     4008    }  & \cellformatrW{  2004      } & \cellformatlW{\bf 2--2000 }\\
\cellformatrW{A3} & \cellformatlW{     10    } & \cellformatrW{\bf 2--1024} & \cellformatlW{\bf 160--81920} & \cellformatrW{    40      } & \cellformatlW{   60\Mark2 }\\
\cellformatrW{A4} & \cellformatlW{     10    } & \cellformatrW{      50   } & \cellformatlW{     4000    }  & \cellformatrW{    40      } & \cellformatlW{\bf 80--1200}\\
\hline
\multicolumn{6}{c}{\vspace*{-0.3cm}}\\
%%%%%%%%%%%%% SECOND PART OF THE TABLE %%%%%%%%%%%%%%%%%%%%%%%%
\hline
\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}\\
\cellformatrG{}&
\cellformatlG{\multirow{-2}{1.6cm}{\centering\bf FFT size\Mark3}} & 
\cellformatrG{\multirow{-2}{*}{\centering\it\#Inputs}} & 
\cellformatlG{\multirow{-2}{*}{\centering\it \#Nodes\Mark1}} & 
\cellformatrG{\multirow{-2}{1.8cm}{\centering\it Critical path}}&
\cellformatlG{\multirow{-2}{2cm}{\centering\bf Latency ($T_{iter}$)}}\\
\cellformatrG{\multirow{-3}{2.2cm}{\centering Benchmark: FFT}}& 
\cellformatlG{\footnotesize$(1)$} & 
\cellformatrG{\footnotesize$(2)=2^{(1)}$} & 
\cellformatlG{\footnotesize$(3)=10\cdot(1)\cdot (2)$} & 
\cellformatrG{\footnotesize$(4)=4\cdot (1)$} & 
\cellformatlG{\footnotesize$(5)$}\\
\hline
\cellformatrW{F1} & \cellformatlW{\bf 1--10} & \cellformatrW{2--1024} & \cellformatlW{\bf 20--102400} &  \cellformatrW{4--40} & \cellformatlW{6--60\Mark2}\\
\cellformatrW{F2} & \cellformatlW{\bf 5} & \cellformatrW{32} & \cellformatlW{1600} & \cellformatrW{20} & \cellformatlW{\bf 40 -- 1500}\\
\hline
\multicolumn{6}{c}{\vspace*{-0.3cm}}\\
% THIRD AND LAST TABLE!!!
\hline
\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}&\cellformatrG{}&\cellformatlG{}\\
\cellformatrG{}&
\cellformatlG{\multirow{-2}{*}{\centering\bf\#Types}} & 
\cellformatrG{\multirow{-2}{*}{\centering\bf \#Nodes}} & 
\cellformatlG{\multirow{-2}{*}{\centering\it \#Networks}} & 
\cellformatrG{\multirow{-2}{1.8cm}{\centering\it Critical path}}&
\cellformatlG{\multirow{-2}{2cm}{\centering\bf Latency ($T_{iter}$)}}\\
\cellformatrG{\multirow{-3}{2.2cm}{\centering Benchmark: Random networks}}& 
\cellformatlG{\footnotesize$(1)$} & 
\cellformatrG{\footnotesize$(2)$} & 
\cellformatlG{\footnotesize$(3)$} &
\cellformatrG{\footnotesize$(4)$} & 
\cellformatlG{\footnotesize$(5)$}\\
\hline
\cellformatrW{R1} & \cellformatlW{3} & \cellformatrW{10--2000} & \cellformatlW{500} &  \cellformatrW{\it variable} & \cellformatlW{\footnotesize$(4)$}\\
\cellformatrW{R2} & \cellformatlW{3} & \cellformatrW{  50    } & \cellformatlW{500} &  \cellformatrW{\it variable} & \cellformatlW{\footnotesize$(4)\times [1;\cdots;20]$}\\
\hline
\multicolumn{6}{c}{\vspace*{-0.3cm}}\\
\multicolumn{6}{l}{\it\Mark1 Excluding constant nodes.}\\
\multicolumn{6}{l}{\it\Mark2 Value kept proportional to the critical path: $(5)=(4)*1.5$.}\\
\multicolumn{6}{l}{\it\Mark3 A size of $x$ corresponds to a $2^x$ point FFT.}\\
\multicolumn{6}{l}{\it Values in bold indicate the parameter being varied.}
\end{tabular}
\end{table}
